Sensitivity of Single-Pulse Radar Detection to Radar State Uncertainty

Mission planners for aircraft operating under threat of detection from ground-based radar systems are often concerned with the probability of detection. Current approaches to path planning in such environments consider the radar state (i.e. radar position and parameters) to be deterministic and known. In practice, there is uncertainty in the radar state which induces uncertainty in the probability of detection. This paper presents a method to incorporate the uncertainty of the radar state in a single-pulse radar detection model. The method linearizes the radar detection model with respect to the the radar state and uses the linearized models to estimate, to the first order, the variance of the probability of detection. The results in this paper validate the linearization using Monte Carlo analysis and illustrate the sensitivity of the probability of detection to radar state uncertainty.

==> sections/LutRCS.tex <==
\paperplan{LUT RCS}{
    \begin{itemize}
        \item RCS models take many forms
        \item In practice, RCS is measured and provided in LUT
        \item LUT function wrt RCS azimuth and elevation angles
        \item Objective of function fitting - envelope 
        \item Optimization method for polynomial envelope
    \end{itemize}
}


==> sections/RadarParitials.tex <==
This appendix provides equations for partial derivatives that are derived in \cite{costley2022sensitivity} and used in this paper.
The partial derivative of $P_D$ \eqref{eq:pd_approx} with respect to the aircraft state is given by 
\begin{equation}
    A_{Pa} = \frac{\partial P_D}{\partial \mathcal{S}}\begin{bmatrix}\frac{\partial \mathcal{S}}{\partial R}\frac{\partial R}{\partial\boldsymbol{x_{a}}}+\frac{\partial \mathcal{S}} {\partial\sigma_{r}}\frac{\partial\sigma_{r}}{\partial\boldsymbol{x_{a}}}\end{bmatrix} \Bigg\rvert_{\boldsymbol{\bar{x}_a}} 
\end{equation}
where the first three partial derivatives are given by
\begin{gather}
    \frac{\partial P_{D}}{\partial\mathcal{S}} = \frac{\exp\left(-\left(\sqrt{-\ln P_{fa}}-\sqrt{\mathcal{S}+0.5}\right)^2\right)}{2\sqrt{\pi}\sqrt{\mathcal{S}+0.5}} \label{eq:dp_dsnr} \\
    \frac{\partial\mathcal{S}}{\partial R} = -c_r\frac{4 \sigma_r}{kR^{5}} \\
    \frac{\partial R}{\partial\boldsymbol{x_{a}}}  = \begin{bmatrix}\frac{\left(\boldsymbol{p_{a}-p_{r}}\right)^\intercal}{||\boldsymbol{p_{a}-p_{r}}||_{2}} & \boldsymbol{0_{1x3}}\end{bmatrix}.
\end{gather}

The remaining expressions provide the partial derivative of $S$ with respect to the aircraft state.
The first partial derivative is given by
\begin{align}
    \frac{\partial\mathcal{S}}{\partial\sigma_{r}} & = c_r\frac{1}{kR^{4}}.
\end{align}
The partial derivative of the RCS with respect to the aircraft state is given by
\begin{align}
    \partiald{\sigma_r}{\boldsymbol{x_a}} = \partiald{\sigma_r}{\lambda} \partiald{\lambda}{\boldsymbol{x_a}} + \partiald{\sigma_r}{\phi} \partiald{\phi}{\boldsymbol{x_a}}
\end{align}
where $\partiald{\sigma_r}{\lambda}$ and $\partiald{\sigma_r}{\phi}$ for the ellipsoid model are given in \eqref{eq:dsig_dlam} and \eqref{eq:dsig_dphi}.
The partial derivative of the RCS azimuth and elevation angles are given by 
\begin{eqnarray}
    \partiald{\lambda}{\boldsymbol{x_a}} &=& \partiald{\lambda}{\boldsymbol{\rho_r^b}} \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{x_a}} \\
    \partiald{\phi}{\boldsymbol{x_a}} &=& \partiald{\phi}{\boldsymbol{\rho_r^b}} \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{x_a}}
\end{eqnarray}
where 
\begin{equation}
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{x_a}} = \begin{bmatrix} \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{p_a^n}} & \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}} \end{bmatrix}.
\end{equation}

The partial derivative of $\boldsymbol{\rho_r^b}$ with respect to the aircraft position in the NED frame is given by
\begin{equation}
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{p_a^n}} = -R_n^b
\end{equation}
where $R_n^b$ is defined in \eqref{eq:DCM_zyx}. The partial derivative of $\boldsymbol{\rho_r^b}$ with respect to the aircraft orientation is given by
\begin{equation}
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}} = \begin{bmatrix} \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{11} & \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{12} & \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{13} \\
        \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{21} & \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{22} & \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{23} \\
        \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{31} & \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{32} & \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{33} \end{bmatrix}
\end{equation}
where
\begin{eqnarray}
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{11} &=& -(C{\phi_a} S{\psi_a} - C{\psi_a} S{\phi_a} S{\theta_a})p_{\Delta d} \nonumber \\
            && \quad -(S{\phi_a} S{\psi_a} + C{\phi_a} C{\psi_a} S{\theta_a})p_{\Delta e} \\
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{12} &=& C{\psi_a} S{\theta_a} p_{\Delta n} - C{\psi_a} C{\theta_a} S{\phi_a} p_{\Delta e} \nonumber  \\
            && \quad - C{\phi_a} C{\psi_a} C{\theta_a} p_{\Delta d} \\
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{13} &=& (C{\phi_a} C{\psi_a} + S{\phi_a}S{\psi_a}S{\theta_a})p_{\Delta e} \nonumber  \\
            && \quad - (C{\psi_a} S{\phi_a} - C{\phi_a} S{\psi_a} S{\theta_a}) p_{\Delta d} \nonumber  \\
            && \quad + C{\theta_a} S{\psi_a} p_{\Delta n} \\
%
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{21} &=& (C{\phi_a} C{psi_a} + S{\phi_a} S{\psi_a} S{\theta_a}) p_{\Delta d} \nonumber \\
        && \quad + (C{\psi_a} S{\phi_a} - C{\phi_a} S{\psi_a} S{\theta_a}) p_{\Delta e} \\
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{22} &=& S{\psi_a} S{\theta_a} p_{\Delta n} - C{\phi_a} C{\theta_a} S{\psi_a} p_{\Delta d} \nonumber \\
        && \quad - C{\theta_a} S{\phi_a} S{\psi_a} p_{\Delta e} \\
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{23} &=& (C{\phi_a} S{\psi_a} - C{\psi_a}S{\phi_a}S{\theta_a})p_{\Delta e} \nonumber \\
        && \quad - (S{\phi_a} S{\psi_a} + C{\phi_a}C{\psi_a}S{\theta_a}) p_{\Delta d} \nonumber \\
        && \quad - C{\psi_a} C{\theta_a} p_{\Delta n} \\
%
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{31} &=& C{\theta_a} S{\phi_a} p_{\Delta d} - C{\phi_a} C{\theta_a} p_{\Delta e} \\
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{32} &=& C{\theta_a} p_{\Delta n} + C{\phi_a} S{\theta_a} p_{\Delta d} + S{\phi_a} S{\theta_a} p_{\Delta e}   \\
    \partiald{\boldsymbol{\rho_r^b}}{\boldsymbol{\Theta_a}}_{32} &=& 0
\end{eqnarray}
and
\begin{eqnarray}
    \boldsymbol{p_\Delta^n} &=& \boldsymbol{p_r^n}-\boldsymbol{p_a^n} \\
        &=& \begin{bmatrix} p_{\Delta n} & p_{\Delta e} & p_{\Delta d} \end{bmatrix}^\intercal.
\end{eqnarray}

